Measuring the Internet during Covid-19 to Evaluate Work-from-Home

Covid-19 has radically changed our lives, with many governments and businesses mandating work-from-home (WFH) and remote education. However, work-from-home policy is not always known globally, and even when enacted, compliance can vary. These uncertainties suggest a need to measure WFH and confirm actual policy implementation. We show new algorithms that detect WFH from changes in network use during the day. We show that change-sensitive networks reflect mobile computer use, detecting WFH from changes in network intensity, the diurnal and weekly patterns of IP address response. Our algorithm provides new analysis of existing, continuous, global scans of most of the responsive IPv4 Internet (about 5.1M /24 blocks). Reuse of existing data allows us to study the emergence of Covid-19, revealing global reactions. We demonstrate the algorithm in networks with known ground truth, evaluate the data reconstruction and algorithm design choices with studies of real-world data, and validate our approach by testing random samples against news reports. In addition to Covid-related WFH, we also find other government-mandated lockdowns. Our results show the first use of network intensity to infer-real world behavior and policies.

==> Makefile <==

.PHONY: all pdf FORCE_MAKE
all pdf:: paper.pdf

%.pdf: %.tex FORCE_MAKE
	latexmk -pdf $<

clean::
	latexmk -c

abstract.txt: paper.tex
	< $< sed -e '1,/begin{abstract}/d' -e '/end{abstract}/,$$d' -e 's/%.*$$//' -e 's/^[ 	]*//' | \
	  fmt >$@

strip_comments:
	/home/johnh/BIN/uncommentify -l tex paper.tex >CLEAN/paper.tex


